Certified Guidance for Planning with Deep Generative Models

Deep generative models, such as generative adversarial networks and diffusion models, have recently emerged as powerful tools for planning tasks and behavior synthesis in autonomous systems. Various guidance strategies have been introduced to steer the generative process toward outputs that are more likely to satisfy the planning objectives. These strategies avoid the need for model retraining but do not provide any guarantee that the generated outputs will satisfy the desired planning objectives. To address this limitation, we introduce certified guidance, an approach that modifies a generative model, without retraining it, into a new model guaranteed to satisfy a given specification with probability one. We focus on Signal Temporal Logic specifications, which are rich enough to describe nontrivial planning tasks. Our approach leverages neural network verification techniques to systematically explore the latent spaces of the generative models, identifying latent regions that are certifiably correct with respect to the STL property of interest. We evaluate the effectiveness of our method on four planning benchmarks using GANs and diffusion models. Our results confirm that certified guidance produces generative models that are always correct, unlike existing guidance methods that are not certified.

==> sections/algorithm.tex <==
\subsection{Algorithm}\label{sec:algorithm}

In Algorithm~\ref{alg:prob_sat}, we illustrate our framework for lower-bounding $P_\property$. In lines 1–12 the algorithm computes $B$, which is the union of $\property$-satisfying sets of latent inputs, which is a subset of $\overline{B}$, the maximal $\property$-satisfying set (see Definition~\ref{def:sat_set}).In general, $\overline{B}$ is not a connected set. Hence, we build $B$ as a union of hyper-rectangles (line 12), each of which is $\property$-satisfying. Each candidate $\property$-satisfying hyper-rectangle is generated as follows: we sample a random latent input $\latentvar_0^i$ (line 6) from which we start a GD-search of $\latentvar_*^i$ (line 7), a local optimum. This process is repeated $\nballs$ times to generate multiple $\property$-satisfying rectangles in disconnected regions of the latent space. In lines 8-11 we check if the given hyper-rectangle is $\property$-satisfying by using Auto-LiRPA, we also check the non-overlapping property (lines 9 and 12). We iteratively increment $\varepsilon$ until both the $\property$-satisfying and the non-overlapping properties are met (lines 9-11). All $\property$-satisfying non-overlapping hyper-rectangles are added to $B$ (lines 12-13).
Finally, in lines 14–18, by employing Corollary~\ref{cor:lb}, we compute a lower bound for $P_\property$.


\begin{algorithm}
\caption{Probabilistic Satisfaction for DGM}\label{alg:prob_sat}
\begin{algorithmic}[1]
\State \textit{Input:} Generator $\gen$, STL property $\property$, $M$ (max number of perturbation balls, $\varepsilon_0$.

\State \textit{Output:} Lower bound for the satisfaction probability $P_\property$.

\State $B \gets \emptyset$
\For{$i=1:M$}
    \State $\varepsilon \gets \varepsilon_0$
    \State $\latentvar_0^i \sim p( \latentvar)$
    \Comment{\texttt{Gradient descent optimization over latent variables starting in $\latentvar_0^i$}}
    \State $\latentvar_*^i \gets \texttt{GD}(-r^\property_\weights(\latentvar),\latentvar_0^i,\gamma)$ 
    \State $\underline{b}_\property,\overline{b}_\property \gets \texttt{Verifier}\left(r_\weights(\latentvar), \mathcal{B}(\latentvar_*^i,\varepsilon)\right)$ \Comment{\texttt{Lower and Upper bounds over Boolean Satisfaction $\rchi_\property$}}
    \While{$\underline{b}_\property = 1\ \land \mathcal{B}(\latentvar_*^i,\varepsilon)\cap B = \emptyset$}
        \State $\varepsilon \gets \varepsilon + \Delta\varepsilon$
        \State $\underline{b}_\property,\overline{b}_\property \gets \texttt{Verifier}\left(r_\weights(\latentvar), \mathcal{B}(\latentvar_*^i,\varepsilon)\right)$
    \EndWhile
    \If{$\underline{b}_\property = 1\land \mathcal{B}(\latentvar_*^i,\varepsilon)\cap B = \emptyset$}
    \State $B\gets B\cup   \mathcal{B}(\latentvar_*^i,\varepsilon)$
    \EndIf
    

\EndFor

\State $p\gets 0.0$

\If{$B\ne\emptyset$}
\For{$d\gets 1:M'$} \Comment{\texttt{$M'$: \# hyper-rectangles in B}}
\State $l^d, u^d \gets \texttt{GetBall}(B,d)$
\State $p\gets p+\prod_{i=1}^\latentdim \frac{1}{2}\left(
erf\left(-\frac{l^d_i}{\sqrt{2}}\right)-erf\left(-\frac{u^d_i}{\sqrt{2}}\right)
\right)$
\EndFor

\EndIf
\end{algorithmic}
\end{algorithm}
